Bootstrapping the relativistic two-body problem

We describe the formalism to compute gravitational-wave observables for compact binaries via the effective field theory framework in combination with modern tools from collider physics. We put particular emphasis on solving the "multi-loop" integration problem via the methodology of differential equations and expansion by regions. This allows us to "bootstrap" the two-body relativistic dynamics in the Post-Minkowskian (PM) expansion from boundary data evaluated in the near-static (soft) limit. We illustrate the procedure with the derivation of the total spacetime impulse in the scattering of non-spinning bodies to 4PM (three-loop) order, i.e. ${\cal O}(G^4)$, including conservative and dissipative effects.

==> diagsSeff.tex <==
\centering
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-0.9, 0) -- (0.9,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-0.9, -2) -- (0.9,-2);
  \draw[graviton] (0,-2) -- (0,0);
  \fill[color=internationalorange] (0,0) circle (1.5pt);
  \fill[color=internationalorange] (0,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(1)$};
\end{tikzpicture}
\hspace{8mm}
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.0, 0) -- (1.0,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.0, -2) -- (1.0,-2);
  \draw[graviton] (-0.7,0) -- (0,-1);
  \draw[graviton] (0.7,0) -- (0,-1);
  \draw[graviton] (0,-2) -- (0,-1);
  \fill[color=internationalorange] (0,-2) circle (1.5pt);
  \fill[color=internationalorange] (-0.7,0) circle (1.5pt);
  \fill[color=internationalorange] (0.7,0) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(2)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (0,-2) -- (0,-1);
  \draw[graviton] (-0.8,0) -- (0,-1);
  \draw[graviton] (0.8,0) -- (0,-1);
  \draw[graviton] (0,0) -- (-0.32,-0.59);
  \fill[color=internationalorange] (0,-2) circle (1.5pt);
  \fill[color=internationalorange] (-0.8,0) circle (1.5pt);
  \fill[color=internationalorange] ( 0.8,0) circle (1.5pt);
  \fill[color=internationalorange] ( 0.0,0) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(3)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.7,0) -- (0,-0.7);
  \draw[graviton] (0.7,0) -- (0,-0.7);
  \draw[graviton] (-0.7,-2) -- (0,-1.3);
  \draw[graviton] (0.7,-2) -- (0,-1.3);
  \draw[graviton] (0,-0.7) -- (0,-1.3);
  \fill[color=internationalorange] (-0.7,0) circle (1.5pt);
  \fill[color=internationalorange] (0.7,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.7,-2) circle (1.5pt);
  \fill[color=internationalorange] (0.7,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(4)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.0, 0) -- (1.0,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.0, -2) -- (1.0,-2);
  \draw[graviton] (-0.75,0) -- (-0.25,-1);
  \draw[graviton] (0.75,0) -- (0.25,-1);
  \draw[graviton] (-0.75,-2) -- (-0.25,-1);
  \draw[graviton] (0.75,-2) -- (0.25,-1);
  \draw[graviton] (-0.25,-1) -- (0.25,-1);
  \fill[color=internationalorange] (-0.75,0) circle (1.5pt);
  \fill[color=internationalorange] (0.75,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.75,-2) circle (1.5pt);
  \fill[color=internationalorange] (0.75,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(5)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (0,-2) -- (0,-1);
  \draw[graviton] (-0.8,0) -- (0,-1);
  \draw[graviton] (0.8,0) -- (0,-1);
  \draw[graviton] (0,0) -- (0,-1);
  \fill[color=internationalorange] (0,-2) circle (1.5pt);
  \fill[color=internationalorange] (-0.8,0) circle (1.5pt);
  \fill[color=internationalorange] ( 0.8,0) circle (1.5pt);
  \fill[color=internationalorange] ( 0.0,0) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(6)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.7,0) -- (0,-1);
  \draw[graviton] (0.7,0) -- (0,-1);
  \draw[graviton] (-0.7,-2) -- (0,-1);
  \draw[graviton] (0.7,-2) -- (0,-1);
  \fill[color=internationalorange] (-0.7,0) circle (1.5pt);
  \fill[color=internationalorange] (0.7,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.7,-2) circle (1.5pt);
  \fill[color=internationalorange] (0.7,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(7)$};
\end{tikzpicture}

\vskip 5mm
\centering
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.9,0) -- (0,-1);
  \draw[graviton] (0.9,0) -- (0,-1);
  \draw[graviton] (-0.3,0) -- (0,-1);
  \draw[graviton] (0.3,0) -- (0,-1);
  \draw[graviton] (0,-2) -- (0,-1);
  \fill[color=internationalorange] (0,-2) circle (1.5pt);
  \fill[color=internationalorange] (-0.9,0) circle (1.5pt);
  \fill[color=internationalorange] (0.9,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.3,0) circle (1.5pt);
  \fill[color=internationalorange] (0.3,0) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(8)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.9,0) -- (0,-1);
  \draw[graviton] (0.9,0) -- (0,-1);
  \draw[graviton] (0.3,0) -- (0,-1);
  \draw[graviton] (-0.3,0) -- (-0.41,-0.55);
  \draw[graviton] (0,-2) -- (0,-1);
  \fill[color=internationalorange] (0,-2) circle (1.5pt);
  \fill[color=internationalorange] (-0.9,0) circle (1.5pt);
  \fill[color=internationalorange] (0.9,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.3,0) circle (1.5pt);
  \fill[color=internationalorange] (0.3,0) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(9)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (0,-2) -- (0,-1);
  \draw[graviton] (-0.9,0) -- (0,-1);
  \draw[graviton] (0.9,0) -- (0,-1);
  \draw[graviton] (-0.35,0) -- (-0.35,-0.61);
  \draw[graviton] (0.2,0) -- (-0.35,-0.61);
  \fill[color=internationalorange] (0,-2) circle (1.5pt);
  \fill[color=internationalorange] (-0.9,0) circle (1.5pt);
  \fill[color=internationalorange] ( 0.9,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.35,0) circle (1.5pt);
  \fill[color=internationalorange] ( 0.2,0) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(10)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (0,-2) -- (0,-1);
  \draw[graviton] (-0.9,0) -- (0,-1);
  \draw[graviton] (0.9,0) -- (0,-1);
  \draw[graviton] (-0.3,0) -- (-0.53,-0.4);
  \draw[graviton] (0.3,0) -- (-0.26,-0.7);
  \fill[color=internationalorange] (0,-2) circle (1.5pt);
  \fill[color=internationalorange] (-0.9,0) circle (1.5pt);
  \fill[color=internationalorange] ( 0.9,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.3,0) circle (1.5pt);
  \fill[color=internationalorange] (0.3,0) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(11)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (0,-2) -- (0,-1);
  \draw[graviton] (-0.9,0) -- (0,-1);
  \draw[graviton] (0.9,0) -- (0,-1);
  \draw[graviton] (-0.25,0) -- (-0.4,-0.56);
  \draw[graviton] (0.25,0) -- (0.4, -0.56);
  \fill[color=internationalorange] (0,-2) circle (1.5pt);
  \fill[color=internationalorange] (-0.9,0) circle (1.5pt);
  \fill[color=internationalorange] ( 0.9,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.25,0) circle (1.5pt);
  \fill[color=internationalorange] (0.25,0) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(12)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.8,0) -- (0,-1);
  \draw[graviton] (0.8,0) -- (0,-1);
  \draw[graviton] (0,0) -- (0,-1);
  \draw[graviton] (-0.7,-2) -- (0,-1);
  \draw[graviton] (0.7,-2) -- (0,-1);
  \fill[color=internationalorange] (-0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0, 0) circle (1.5pt);
  \fill[color=internationalorange] (-0.7, -2) circle (1.5pt);
  \fill[color=internationalorange] (0.7, -2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(13)$};
\end{tikzpicture}

\vskip 5mm
\centering
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.9,0) -- (0,-1.1);
  \draw[graviton] (0.9,0) -- (0,-1.1);
  \draw[graviton] (0,0) -- (-0.38,-0.63);
  %
  \draw[graviton] (-0.8,-2) -- (0,-1.1);
  \draw[graviton] (0.8,-2) -- (0,-1.1);
  \fill[color=internationalorange] (-0.9,0) circle (1.5pt);
  \fill[color=internationalorange] (0.9,0) circle (1.5pt);
  \fill[color=internationalorange] (0,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.8,-2) circle (1.5pt);
  \fill[color=internationalorange] (0.8,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(14)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.8,0) -- (0,-0.7);
  \draw[graviton] (0.8,0) -- (0,-0.7);
  \draw[graviton] (0,0) -- (0,-1.3);
  %
  \draw[graviton] (-0.8,-2) -- (0,-1.3);
  \draw[graviton] (0.8,-2) -- (0,-1.3);
  \fill[color=internationalorange] (-0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.8,-2) circle (1.5pt);
  \fill[color=internationalorange] (0.8,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(15)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.8,0) -- (0,-0.75);
  \draw[graviton] (0.8,0) -- (0,-0.75);
  \draw[graviton] (0,0) -- (-0.37,-0.42);
  %
  \draw[graviton] (0, -0.75) -- (0, -1.35);
  %
  \draw[graviton] (-0.8,-2) -- (0,-1.35);
  \draw[graviton] (0.8,-2) -- (0,-1.35);
  \fill[color=internationalorange] (-0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.8,-2) circle (1.5pt);
  \fill[color=internationalorange] (0.8,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(16)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.8, 0) -- (-0.3, -1);
  \draw[graviton] (0.8, 0) -- (0.35, -1);
  \draw[graviton] (0,0) -- (-0.3, -1);
  %
  \draw[graviton] (-0.3, -1) -- (0.35, -1);
  %
  \draw[graviton] (-0.8, -2) -- (-0.3, -1);
  \draw[graviton] (0.8, -2) -- (0.35, -1);
  \fill[color=internationalorange] (-0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.8,-2) circle (1.5pt);
  \fill[color=internationalorange] (0.8,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(17)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
  \draw[graviton] (-0.8, 0) -- (-0.35, -1);
  \draw[graviton] (0.8, 0) -- (0.35, -1);
  \draw[graviton] (0,0) -- (0, -1);
  %
  \draw[graviton] (-0.35, -1) -- (0.35, -1);
  %
  \draw[graviton] (-0.8, -2) -- (-0.35, -1);
  \draw[graviton] (0.8, -2) -- (0.35, -1);
  \fill[color=internationalorange] (-0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.8,-2) circle (1.5pt);
  \fill[color=internationalorange] (0.8,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(18)$};
\end{tikzpicture}~~
%%
\begin{tikzpicture}[scale=1]
  %\draw[line width=1.0pt] (-1.1, 0) -- (1.1,0);  % node[right] {$1$};
  %\draw[line width=1.0pt] (-1.1, -2) -- (1.1,-2);
   \draw[graviton] (0.8, 0) -- (0.35, -1.1);
  \draw[graviton] (-0.25,-1.1) -- (-0.35,-0.6);
  \draw[graviton] (-0.8, 0) -- (-0.35,-0.6) -- (0, 0);
  %
  \draw[graviton] (-0.25, -1.1) -- (0.35, -1.1);
  %
  \draw[graviton] (-0.8, -2) -- (-0.25, -1.1);
  \draw[graviton] (0.8, -2) -- (0.35, -1.1);
  \fill[color=internationalorange] (-0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0.8,0) circle (1.5pt);
  \fill[color=internationalorange] (0,0) circle (1.5pt);
  \fill[color=internationalorange] (-0.8,-2) circle (1.5pt);
  \fill[color=internationalorange] (0.8,-2) circle (1.5pt);
  %\fill[yshift=-25mm] (0,0) circle (0) node[] {$(19)$};
\end{tikzpicture}


==> widebar.tex <==
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother

